Towards Interpretable Sequence Continuation: Analyzing Shared Circuits in Large Language Models

While transformer models exhibit strong capabilities on linguistic tasks, their complex architectures make them difficult to interpret. Recent work has aimed to reverse engineer transformer models into human-readable representations called circuits that implement algorithmic functions. We extend this research by analyzing and comparing circuits for similar sequence continuation tasks, which include increasing sequences of Arabic numerals, number words, and months. By applying circuit interpretability analysis, we identify a key sub-circuit in both GPT-2 Small and Llama-2-7B responsible for detecting sequence members and for predicting the next member in a sequence. Our analysis reveals that semantically related sequences rely on shared circuit subgraphs with analogous roles. Additionally, we show that this sub-circuit has effects on various math-related prompts, such as on intervaled circuits, Spanish number word and months continuation, and natural language word problems. Overall, documenting shared computational structures enables better model behavior predictions, identification of errors, and safer editing procedures. This mechanistic understanding of transformers is a critical step towards building more robust, aligned, and interpretable language models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_texs/0_todo.tex <==

% \TODO{Just Finished and To Do Next}

% \textbf{Overall Plan (Now):}
% Find common circuits for more numerical tasks (cont, >, mod, etc)

\textbf{Just Finished}

\begin{itemize}
    \item Improved path patching. plotted distribution of path patch edge thresholds for each end-head to get avg for all
    \item Get circuits for multiple tasks (months, words, etc) with lower performance to find sub-circuits with greater-than.
\end{itemize}

\textbf{Working on now: } The corruption type used in auto ablation and path patching tells the functionality; see docstring circuit

Add MLPs to circuit. Logit/Tuned Lens, ACDC.

\textbf{Later: }
At what threshold does it lose shared sub-circuits with greater-than?

Head 9.1 seems to be common in gpt2-small, but does it work the same in each circuit?

Get SVD as perc of (l,h,dir), NOT (l,h). this is bc each dir has its own feature, not (l,h). In svd, don’t just search for “digit” dirs, but “next” or “change” dirs

More detailed figure captions

(\textbf{AIM: trim paper to two-col 8 pages, with long Appendix).} Rmnv expms w/ least useful results; structure github repo better (remove most notebooks) 

----------------

% \TODO{Based on "Start with an outline rather than full text." in "HOW TO ML FB" doc. Write a paragraph for each section}

Table of Contents: (for draft organization purposes only; remove in final submission version)

\begin{enumerate}
    \item Introduction
    \item Background

    \item Related Work \hl{decide by: https://academia.stackexchange.com/questions/13270/is-it-better-to-write-related-work-at-the-start-or-in-the-end}
        \begin{enumerate}
            \item A lot of "methodology" was repeated before, so they can be described in related work?
        \end{enumerate}
    
    \item Methodology
    \begin{enumerate}
        \item Connectivity Methods
        \begin{enumerate}
            \item Path Patching, Automated Ablation
        \end{enumerate}
        \item Functionality Methods
        \begin{enumerate}
            \item Logit Lens / OV Scores (copy, next)
            \item SVD 
            \item N2G / Neuroscope
        \end{enumerate}
    \end{enumerate}
    \item Experimental Results
    \begin{enumerate}
        \item Model, Dataset, Similar Task Types
        \item Shared Circuits of Similar Tasks
        \begin{enumerate}
            \item Connectivity, figure of circuit hypotheses
            \item Functionality  (pure + among words for attention patterns)
        % \item \hl{(May have time; else edit title to be "Similar Numerical Tasks")}: Shared circuit between subject tasks
        % \item \hl{(Likely will not have time; save for later)}: Shared circuit for adjectives, type hierarchies (animals, etc), etc.
    \end{enumerate}
\end{enumerate}
\item \hl{(To Do)}: Model editing
\item Conclusion
\item Appendix
\end{enumerate}

==> old_texs/mlps.tex <==
\subsection{MLP Analysis}

% [This section may be rmv / move to appendix as it doesn't directly interact with hypothesized circuit]

We utilize activation patching on individual neurons to find important neurons, as displayed in Figure \ref{mlp_actvpath}. Using multi-prompts for digits, we look at L9 and L10 to find two that stand out as “number neurons” (their contribution is partial, so combinations of neurons are likely involved):
\begin{itemize}
\item Layer 9: 934 
\item Layer 10: 1721 
\end{itemize}

\begin{figure}[H]
% \begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{plots/fig 7.pdf}
  \caption{Activation Patching by Neuron for L10. Neuron 1721 stand out as having more than 0.2 patch improvement
}
\label{mlp_actvpath}
\end{figure}

Neuroscope supports these findings by showing its strong activations near number-type tokens, as seen in Figure \ref{fig:neuroscope}.

\begin{figure}[H]
% \begin{figure}[ht]
  \centering
  \includegraphics[scale=0.4]{plots/maxactv.pdf}
  \caption{A max activating example from the dataset for L10, N1721
}
\label{fig:neuroscope}
\end{figure}

\subsubsection{SVD Analysis}

To lessen the amount of API calls, we note that \cite{millidge2022singular} stored whether a singular vector was interpretable by the model or not. Thus, we only consider vectors that were already labeled in the previous study as interpretable.

MLP weight matrix singular vectors are stated to be more polysemantic and less interpretable than attention head OV weight matrix singular vectors. As such, a concept must share a direction with other concepts. We analyze MLP input weight matrices.

We note that X out of X, or around X\%, singular directions are labeled as interpretable, and X out of X, or around X\%, of these interpretable directions are found to correspond to [seq type] concepts.

==> old_texs/model2model.tex <==
\subsection{Model-To-Model Comparison}

In previous sections, we compared components that activated for analogous input sequences. In this section, we use the same input sequences on different models to see if there are analogous circuit components between models.

\subsubsection{Comparison to GPT-2 Medium}

We compare running the input sequence “2 4 6 8 10 12” on both  GPT-2 Small and GPT-2 Medium. Attention heads that attend to tokens further back than previous token are of interest to observe if sequences are recognized based on members of the sequence that are further back than the previous token.

We notice that in GPT-2 Medium, head 11.4 attends from the last token "12" to token “6”, which is three tokens back. This is similar to head 6.1 in GPT-2 Small attends from the last token "four" to token "two", which is two tokens back.

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{plots/6.1 small vs 11.4 med.pdf}
  \caption{(a) Head 6.1 for GPT-2 Small vs (b) Head 11.4 for GPT-2 Medium
}
\end{figure}

Attention Head Patching discovers that GPT-2 Medium has a head 19.1 that is very important. It may be the case that 9.1 from Small and 19.1 from Medium perform similar functions, as both are very important late heads. [show figure].

[ Future plans to do: Show that these sub-circuit components are analogous across models by showing knocking these sub-circuits will result in analogous performance changes. Not only that, but combos of sub-circuits knocked out will have analogous effects, both when out and when restored. This may be saved for a follow-up paper]

==> templates/algo_templ.tex <==
\begin{algorithm}[!thbp]
 \rule{\linewidth}{.5pt}

 \begin{flushleft}
\emph{Input:} List of neurons

\emph{Output:} Subset of neurons
\end{flushleft}

\begin{small}

\algsetup{linenodelimiter=.}
  \begin{algorithmic}[1]

\STATE test

\end{algorithmic}

\end{small}

\caption{Algorithm {\em
FindNeuronSubset}}
\label{alg}

\end{algorithm}

==> texs/z.futurework.tex <==
\section{Differentiating Intervaled Sequences (by features?)}

Examine how ablating, altering, and steering (small) sequence continuation circuits affects cross-domain mathematical behavior such as sequence reasoning, greater-than, addition, etc. Look at models with the ability to do reasoning well. 

\subsection{Transferring to foreign language math abilities}
\textbf{Perhaps the model doesn’t know Spanish inherently, but it CAN map one to uno. Perhaps we can steer it during reasoning to “know” a bit of Spanish. Get activation additions to steer across languages (experiments so far: llama-2 can reason less-than, but is limited in only knowing up to uno to seis in spanish. can we 'bind' it to know siete, 7, using the mapping found in Gould et al? Figure out its existing english vs spanish counting space relations and modify it.}

Discuss related work on english to chinese/french mech interp for llama-2: \cite{wendler2024llamas}

Analogous steering across languages: starting with sequences, llama-2 is noted to map numbers to both English and Spanish First, we show that the model can do math reasoning in English, but not in Spasnih. Then, we take an English prompt that can do math reasoning, and just steer the english numbers into Spanish, adn see what happens (perhaps it can now reason in Spanish too)

Requires more thought- this steering should not be too narrow. If we just change "5" into "cinco", that's the same as just replacing it in the prompt, and it will fail this reasoning. We need to find a more general "activation addition" that's like (Turner et al.) where it changes the entire "general" generation. Actually, we should look for word problems that are not just "next token" then, but more "less rigorous" generation. 
Or, just experiment and try to steer 5 into cinco, maybe it will work. This is not using cinco directly, but a steering feature/vector, so it's not the same as "just replacing it". We are just injecting some "spanish flair". We hypothesize this can work because in (Wendler et al.), they state: “The machine, so to
say, thinks in English and translates the conversation at the last moment into Estonian” (Piir, 2023). This would be similar to what we're doing, with the steering being the "last moment" that adds on to the already English thinking. The difference is that the spanish reasoning prompt doesn't use english reasoning, but english reasoning + spanish steering does use it.

Based on (Wendler et al.), the layer to steer is crucial. "Paths first pass through the English cluster, and only later reach the Chinese cluster. Taken together, the emerging picture is that, when translating a German word to Chinese, Llama-2 takes a “detour” through an English subspace." Find this English subspace and figure out how to steer to other languages when it comes to sequence continuation and similar mathematical tasks (greater than, etc).

Notably, we should check if the spanish continuation in llama-2 uses the sequence detection and sequence continaution heads in llama-2. Also, MLP 9 is important in gpt-2; find its analog in llama-2. If we focus on llama-2, we work with just 1 model, since gpt-2 small can't do spanish seq cont.

Secondary: we introduce expanding this space of associations by attempting to replace one association with another by steering, similar to paris to seattle. Actually this doesn't make much sense when steering bc we arent editing weights; the first goal makes more sense for steering.  [this will take a lot more thinking of how to do]. 

We use English - Natural Numbers - Spanish as the domains (in contrast to ranks - nums - months in Gould et al). Then, we take steering vectors and decompose them to find features. 

the reason why we find the circuit using these inputs is because using the prompts is too specific; we want a general circuit that these prompts share. running all of them is too expensive and hard to evaluate (cannot use logit diff or KL div, which are more rigorous than ‘looking at generation’). 

These sequential behavior prompts are not about math reasoning, but are about indirectly using the concept of sequence reasoning to make decisions. Knowing what is in what order. Eg) Kate is first, Beth is second. Who should the award be given to and why?

Previous work has shown that intervening on language specific neurons can alter outputs to generate the probability of the target language occurrence \cite{kojima2024multilingual}. In our work, we take another approach to language translation intervention by steering using features identified for language mapping. \hl{this paper was accepted at naacl 2024, showing the relevancy of this field for the acl confs}

Our work differs from \cite{kojima2024multilingual} because we are looking to find mapping functions (such as by feature steering) from English to another language which go through the natural numbers as an abstraction intermediary. Whereas \cite{kojima2024multilingual} is more general about generating any output as Spanish, we want to specifically target English number words to have them be viewed as Spanish, and using steering interventions at specific layers that show those layers, and not others, are responsible for this mapping. This is similar to the domain-space projection functions from \cite{gould2023successor}.

\citep{gould2023successor} define tokens $T(i,d)$ as composed for both indexing $i$ (the natural number they map to) and domain $d$ (the type of sequence they map to, such as "months") properties. They project a token $T_1(i=a,d=X)$ to its $i=a$ value, and another token $T_2(i=b,d=Y)$ to its $d=Y$ value. They are able to combine these into a new token, $T_3(i=a,d=Y)$. This is possible by finding the common indexing space that both the tokens in the separate domains both share. In our paper, we use languages as domains.
The notation we use above is not what their paper uses, but we may use this notation in our paper

domain-space projection: this finds the features of "months" from say July

domain-space projection (section 3.1 and appendix L) that could go from say "July" to "Month" and it seems they trained a linear maps model to learn how to do this, it looks similar to decomposing activations into SAE features, but it uses a constraint to enforce getting two terms that are index and domain (separately out July into 7 and Month).

They train matrices to map activations to "features" in these spaces, but not with SAEs. 
May find an ALTERNATIVE way to do this mapping, but probably shouldn't focus on this if they did it already. 

NOTE: Gould et al train a model to decompose into index vs domain terms. We can probably just do this. They didn’t put this back in the model and observe the output, though. Their approach is entirely on the output of the successor head, not on the entire model. This is where our work will differ. We can transfer domains then put it back in the model and see how this affects the output. Will the model, previously outputting numbers, now output things related to months? Or letters? They could transfer between numbers and letters. Roman numerals and greek letters. That has implications for different languages encoding numbers. Can we translate between alphabets? Spanish numbers (uno dos tres)? With the entire model, we get more versatile outputs to build upon Gould et al.

\textbf{Interval sequences: eg) Two, Four, Six (larger models like llama-2)
This is good for sparse feature circuits (small paths) to show which parts of circuit differentiates between numerals vs number words. Forget about months- focus on numerals, number words, ranks.
Fibonacci would not have this; focus on intervals instead.}

Fibonacci sequences, decreasing sequences- decompose these into SAE features too. If not, forget about SAE features for this paper for now. 

Non-feature circuits for intervaled sequences (multp 2 seqs, add 2, compare to equations) in larger models. Compare circuits for operations vs for sequences. 

Rather than decompose into features like S.heads paper's constraint (or you can reproduce using that), find actually how the model computes the differences between 1 and one and first. 

Or, how SAE features relate to entity binding. Entity binding. Modify anything to become "sequential". See how featuers change to "bind" something to an entity. 

look for domain + etc features across different layers, not just MLP0

Clustering of any features related to numbers- shapes, etc. let's go further and relate these clusters to each other. and relate these features

feature paths ACROSS models. map and relate circuits across models. don't focus on transfering from one domain to another (already done). \textbf{show analogous features occur in similar places in the circuit} 

focus on two models: gpt2 and pythia. cross-model circuit mapping of feature circuits.
less likely but can try: cross-model patching using features.


\subsection{Feature Circuits to Differentiate 1 vs One}

TBD
